The gradient complexity of linear regression

We investigate the computational complexity of several basic linear algebra primitives, including largest eigenvector computation and linear regression, in the computational model that allows access to the data via a matrix-vector product oracle. We show that for polynomial accuracy, $\Theta(d)$ calls to the oracle are necessary and sufficient even for a randomized algorithm. Our lower bound is based on a reduction to estimating the least eigenvalue of a random Wishart matrix. This simple distribution enables a concise proof, leveraging a few key properties of the random Wishart ensemble.

==> random_matrix_shit.tex <==
%!TEX root = main.tex

\section{Random Matrix}


We begin by collecting facts about a random Wishart matrix:
\begin{prop}[Facts about random wishart matrices]
\end{prop}




\begin{lem}[Regularity Lemma for Random Matrices] Suppose that $(\matM^{(d)})_{d \in \N} \in (\Sym^d)^N$ are a sequence of random matrices such that there exists a constant $q > 0$ and $B \in \R$ for which $\lim_{d \to \infty} \Pr[\|\matM^{(d)}\| \le B] = 1$, and for which, in distribution
\begin{align*}
 d^{q}(\lambda_{d}(\matM^{(d)}), \lambda_{d-1}(\matM^{(d)}) ) \distconv \calD,
\end{align*}
where $\calD$ has density with respect to the Lebsgue measure on $\R^2$. Then, for any $p \in (0,1)$, there exists  $C_1(p)$ and $C_2(p)$ and $d_0(p) \ge C_1(p)^{1/q}$ 
such that for all
\begin{align}
 \forall d \ge d_0(p),\quad \Pr\left[ 2I - \matM^{(d)} \in \EigClass^d(d^{-q}C_1(p),C_2(p),2+B) \right] \ge 1 - p.\label{eq:stuff}
\end{align}
\end{lem}

\begin{lem}[Regularity Lemma for Random Matrices]\label{lem:matrix_regularity} Let $f: \N \to \R$ be an increasing function with $\lim_{d \to \infty} f(d) = \infty$, and $B \ge 2$. Suppose that $(\matM^{(d)})_{d \in \N} \in (\Sympl^d)^{\N}$ are a sequence of random matrices such that $\lim_{d \to \infty} \Pr[\|\matM^{(d)}\| \le B] = 1$, and for which, in distribution
\begin{align*}
f(d)(\lambda_{d}(\matM^{(d)}), \lambda_{d-1}(\matM^{(d)}) ) \distconv \calD,
\end{align*}
where $\calD$ is a probability measure over $\R^2$ such that $\Pr_{(Z_1,Z_2) \sim \calD}[0 < Z_1 < Z_2 ] = 1$. Then, for any $p \in (0,1)$, there exists  $C_1(p)$ and $C_2(p)$ an such that for all
\begin{align}
 \forall d \ge d_0(p),\quad \Pr\left[ 2I - \matM^{(d)} \in \EigClass^d\left(\frac{1}{f(d)}C_1(p),C_2(p),2+B\right) \right] \ge 1 - p.\label{eq:stuff}
 \end{align}
\end{lem}
\begin{thm}[Eigenspacing for the Wishart Law \cite{ramirez2009diffusion}] The sequence $\matM^{(d)} := \frac{1}{d} \matX$ \maxs{normalize?} satisfies the conditions of Lemma~\ref{lem:matrix_regularity} with $f(d) = d^2$ and $B = 5$. 
\end{thm}
\begin{proof} The correctness of the scaling $f(d) = d^2$ and fact that the limiting distribution satisfies $\Pr_{(Z_1,Z_2) \sim \calD}[0 < Z_1 < Z_2 ] = 1$ follows from \citet[Theorem 1]{ramirez2009diffusion}. It is a standard fact that for the Wishart distribution, $\lim_{d \to \infty} \Pr[\|\matM^{(d)}\| \le 4 + \epsilon] = 1$ for any $\epsilon > 0$ (see, e.g. \citet[Exercise 2.1.18]{anderson2010introduction}). 
\end{proof}
\begin{prop}There exists a universal constant  $p_0$ such that, for all $\alpha \in (0,1)$, and all $d \ge d_0(\alpha)$ such that
\begin{align*}
\Pr[\lambda_1(\matM^{(d)}) \ge d^{-2}] \ge p_0 \quad \text{and} \quad \Pr[\lambda_1(\matM^{(d)}) \le \alpha^2 d^{-2}] \ge p_0 \alpha
\end{align*}
\end{prop}
\begin{proof} 
\end{proof}
\maxs{
This bound can be used to conclude that one need $\left(1 - \alpha^2\right)d$-queries for an $\Omega(\alpha)$ probability of correctness. In particular, the number of queries must be arbitarily close to $d$}



\begin{comment}
\subsection{Proof of Lemma~\ref{lem:matrix_regularity}}
First, we prove the first point. Fix $p \in (0,1)$. Since $\Pr_{(Z_1,Z_2) \sim \calD}[0 < Z_1 < Z_2 ] = 1$, there exists a constants $c_1(p)$, $c_2(p)$ such that the open set 
\begin{align*}
E(p):= \left\{(z_1,z_2) \in \R^d: z_1 \in (0,c_2(p)), z_2 - z_1 > c_2(p)\right\}
\end{align*} satisfies $\Pr_{(Z_1,Z_2) \sim \calD}\left[(Z_1,Z_2) \in E(p) \right] \ge 1-\frac{p}{3}$. Since $E(p)$ is open, convergence in distribution implies that for all $d$ which are sufficiently large (as a function of $p$), 
\begin{align*}
\Pr\left[ f(d)(\lambda_{d}(\matM^{(d)}), \lambda_{d-1}(\matM^{(d)}) ) \in E(p) \right] \ge -\frac{p}{3} + \Pr_{(Z_1,Z_2) \sim \calD}\left[ (Z_1,Z_2) \in E(p)\right] \ge 1 - \frac{2p}{3}.
\end{align*}
Moreover, since $\lim_{d \to \infty} \Pr[\|\matM^{(d)}\| \le B] = 1$, we conclude that for all $d$ sufficiently large as functions of $p$, 
\begin{align*}
&\Pr\left[\left\{\|\matM^{(d)}\| \le B\right\} \cap \left\{\lambda_{d}(\matM^{(d)} \in [0,\frac{c_2(p)}{f(d)}] \right\} \cap \left\{\lambda_{d-1} - \lambda_d \ge c_2(p)\right\}\right]\\
&\qquad\ge \Pr\left[ \left\{\|\matM^{(d)}\| \le B\right\} \cap  \left\{f(d)(\lambda_{d}(\matM^{(d)}), \lambda_{d-1}(\matM^{(d)}) ) \in E(p)\right\} \right] \\
&\qquad\ge \Pr\left[   \left\{f(d)(\lambda_{d}(\matM^{(d)}), \lambda_{d-1}(\matM^{(d)}) ) \in E(p)\right\} \right] - \frac{p}{3} \ge 1 - p.
\end{align*}
The lemma now follows by selecting $C_1(p) = c_1(p)$ and $C_2(p) = c_2(p)/c_1(p)$ in the following claim:
\begin{claim} Suppose $\|\matM^{(d)}\|_{\op} \le B$, that $f(d)\lambda_{d}(\matM^{(d)}) \le c_2$ and $f(d)\left(\lambda_{d-1}(\matM^{(d)}) -  \lambda_{d}(\matM^{(d)})\right) \ge c_1$. Then, for all $d \ge f^{-1}(c_2)$, $2I - \matM^{(d)} \in \EigClass^d\left(\frac{1}{f(d)}c_1,\frac{c_2}{c_1},2+B\right)$
\end{claim}
\begin{proof} It is immediate that $\|2I - \matM^{(d)}\|_{\op} \le 2+B$. Moreover, for $d: f(d) \ge c_2$,  $\gap(2-\lambda_1(\matM^{(d)})) = \frac{c_1/f(d)}{2 - \frac{c_2}{f(d)}} \ge c_1/f(d)$.  Finally  $0 \le 2-\lambda_1(\matM^{(d)}) \le \frac{c_2}{f(d)} =  \frac{c_2}{c_1} \gap(2-\lambda_1(\matM^{(d)})) $. 
\end{proof} 
\end{comment}



==> reduction_proofs.tex <==
%!TEX root = main.tex

\section{Reduction Proofs}
\subsection{Proof of Proposition~\ref{prop:reduction}}





\begin{prop}[Reductions between Query Algorithms]\label{prop:reduction} The follow implications hold:

\begin{enumerate}
	%\item If $\Alg$ is an $(\epsilon,\delta)$-correct $\EAA$ over $\Mclass \subset \Sym^d$  with query complexity $T$ , then there exists an $\EEA$ with query complexity $T+1$ which is $(\epsilon,\delta)$-correct over $\Mclass$.
	\item If $\Alg$ is an $(\epsilon,\delta)$-correct $\EAA$ (resp. $\QAA$) over a class $\Mclass$ with query complexity $T$, then for any $p \in \N$, there exists an $(\epsilon,\delta^p)$-correct $\EAA$ (resp. $\QAA$) with query complexity $(T+1)p$. 
	\item 
\end{enumerate}
\end{prop}


\begin{prop}[Shift-and-Invert Reduction]\label{prop:shift_and_invert}
Fix parameters $B \ge 1$, $\alpha > 0, \nu \in (0,1)$ such that $\alpha\nu \le 1$. Furthermore, let $\delta,\epsilon_1 \in (0,1/e)$, and suppose that $d \ge \BigOmegaSt{\log(1/\delta)}$. Let 
\begin{align*}
\epsilon_0 \le \BigOhSt{ \frac{(\alpha \nu)^5}{B^3}\left( \epsilon_1^2 \wedge (d \delta^2 )^{-1}\right)} = 1/\poly\left(\frac{1}{\epsilon_1},d,\frac{1}{\delta_1},\frac{1}{\alpha \nu},B\right).
\end{align*}
 Then if $\Alg$ is an $(\epsilon_0,\delta)$-correct $\QAA$ over $\QuadClass^d(\frac{2B}{\alpha \nu})$, with query complexity $T$, then there exists an $(\epsilon_1,\delta)$ correct $\EAA$ over $\EigClass(\nu,\alpha,B)$ with with query complexity $\BigOh{TL \log L} $ where  $L = \log \frac{dB}{\epsilon_1\delta}$.
\end{prop}

\textbf{Item 1:} Item $1$ follows from letting $\lamhat = \xhat^\top M \xhat$, which can be computed using at most $1$ additional query to $M$. 
\\
\linebreak
\textbf{Item 2:} For the $\EAA$ case, run $p$ independent copies of $\Alg$ to obtain $\vhat^{(1)},\dots,\vhat^{(p)}$. This takes $Tp$ quereis. In the $\EAA$ case, compute $\vhat^{(j)\top}M\vhat$ for $j \in [p]$, using another $T$ queries, and return $\vhat^{(j_*)}$ for $ j_* := \arg\max_{j \in [p]}\vhat^{(j)\top}M\vhat^{(j)}$. Then, 
\begin{align*}
\Pr\left[\vhat^{(j_*)}M\vhat^{(j_*)} \le (1-\epsilon)\lambda_1(M)\right] \le \Pr_{\Alg,M}\left[\vhat^\top M \vhat \le (1-\epsilon)\lambda_1(M)\right]^p \le \delta^p.
\end{align*}

For the $\QAA$ case, obtain $\xhat^{(1)},\dots,\xhat^{(j)}$ indepent solutions with $Tp$ querries, and return $\xhat^{(j_*)}$ for $j_* \in \argmin \frac{1}{2}\xhat^{(j)\top} A \xhat^{(j)} - b^\top x^{(j)} := f_{A,b}(\xhat^{(j)})$; this requires an additional $T$ queries. A standard computation shows that $f_{A,b}(\xhat^{(j)}) = \|\xhat^{(j)} - A^{-1}b\|_A^2 + \min_{x} f_{A,b}(x)$, and thus the same analysis as the $\EAA$ carries through.
\\
\linebreak
\textbf{Item 3:}  For a $p \in \N$ to be chosen shortly, let $\Alg_{\QAA,p}$ denote the $(\epsilon,\delta^p)$-correct algorithm over $\QuadClass(\kappa)$ with query complexity $T(p+1)$, as ensured by Item 2. Observe that if $A$ has condition number $\kappa$, then whenever $\|\xhat - A^{-1}b\|_{A}^2 \le (\frac{1}{e\kappa}) \cdot\lambda_1(A) \|A^{-1}b - x_0\|_2^2$, we have $\|\xhat - A^{-1}b\|^2 \le \frac{1}{\lambda_d(A)\|\xhat - A^{-1}b\|_{A}^2} \le (\frac{1}{e\kappa}) \cdot\frac{\lambda_1(A)}{\lambda_d(A)} \|A^{-1}b - x_0\|_2^2 = \|A^{-1}b - x_0\|_2^2$. Hence, for any $x_0$, $\Alg_{\QAA,p}$ satisfies
\begin{align*}
\Pr_{A,b,x_0,\Alg_{\QAA,p}}\left[\|\xhat - A^{-1}b\|_{2}^2 \le \frac{1}{e}\|x_0 - A^{-1}b\|_{2}^2\right] \ge 1 - \delta^p.
\end{align*}


Let $\Alg_{\QAA}'$ denote the algorithm that restarts $\Alg_{\QAA,p}$ for $R = \ceil{\log(1/\epsilon)} \le \log(e/\epsilon)$-times, using the $r$-th estimate $\xhat^{(r)}$ for the initial point $x_0^{(r+1)}$. Then, $\Alg_{\QAA}'$ makes at most $Tp\log(e/\epsilon) $ queries, and by a union bound, the output $\xhat^{(R)}$ of $\Alg_{\QAA}'$  
\begin{align*}
\Pr\left[\|\xhat^{(R)} - A^{-1}b\|_{A}^2 \le \lambda_1(A)\|\xhat^{(R)} - A^{-1}b\|_{2}^2\right] 
&\le \Pr\left[\|\xhat^{(R)} - A^{-1}b\|_{2}^2 \le \epsilon\|x_0 - A^{-1}b\|_{2}^2\right] \\
&\ge \Pr\left[\|\xhat^{(R)} - A^{-1}b\|_{2}^2 \le e^{-R}\|x_0 - A^{-1}b\|_{2}^2\right] \\
&\ge 1 - R\delta \ge 1 - \log(e/\epsilon)\delta^p.
\end{align*}
Finally tuning $p$ so that $\log(e/\epsilon)\delta^p \le \delta$ proves the result. 



==> wigner_testing.tex <==
%!TEX root = main.tex

\section{Wigner Testing}

Let $\matW^{(d)} \in \R^{d \times d}$ denote a random Wigner matrix, namely $\matW^{(d)} := \frac{1}{\sqrt{2d}}(\matX^{(d)} + \matX^{(d)\top})$, where $\matX_{ij} \iidsim \calN(0,1)$. We will suppress explicit dependence on $d$ when clear from context. 

We shall show that for an appropriate $C_1,C_2$, a $((\dots)\nu^{-3/2},\frac{1}{10},\nu,d)$ EEA can test between the following two hypotheses
\begin{align*}
H_0 :~ \matM = \matW  \quad \text{v.s.} \quad H_1 :~ \matM = (1+\epsilon) \matW,
\end{align*}
via a test of the form $\psi = \I(\lamhat \ge t)$ for a threshold $t = 2 + \Theta(d^{-2/3})$. More precisely, we have the following proposition:
\begin{prop}\label{prop:testing} Fix $p \in (0,1)$ $\Alg$ be any $(d^{-2/3}C_1(p),d^{-2/3}C_2(p),\delta)$-correct, hen, there exists a test $\psi \in \{0,1\}$ which depends only on the output $\xhat$ of $\Alg$ such that, for $\gamma = $
\begin{align}\label{test_eq}
\Pr_{\matW,\Alg}[\psi] + \Pr_{\gamma\matW,\Alg}[1-\psi] \le 2(p + \delta)
\end{align}
\end{prop}



To prove Propsoition~\ref{prop:testing} we first must study the distribution of the top eigenvalue and the eigengap of $\matW^{(d)}$. We begin with the following now-standard result
(see e.g. Universality at the Edge of the Spectrum in Wigner Random Matrices Alexander Soshnikov)
\newcommand{\TWlaw}{\calD_{\mathrm{TW}}}
\begin{thm}[Bi-Variate Tracy Widom Law]\label{thm:tw} There exists a joint density $\TWlaw$ over $\R^2$, which is absolutely continuous with respect to the Lebesgue measure such that $(d^{2/3}(\lambda_1(\matW^{(d)}) - 2,d^{2/3}(\lambda_2(\matW^{(d)}) - 2)) \overset{d \to \infty}{\to} \TWlaw$ in distribution.  
\end{thm}
From this more powerful statement, we can deduce that a certain good event occurs with constant probability:


\newcommand{\query}[1]{\mathsf{v}^{(#1)}}
\newcommand{\Query}[1]{\mathsf{V}^{(#1)}}


By Graham-Schmidt, we may assume that $\query{1},\dots,\query{T}$ are orthonormal. 

%We let $\Query{t} $ denote the matrix whose rows are $[\query{1} | \dots | \query{t}]$, and $I_{t,d}$ denote the matrix $\begin{bmatrix} I_{t} \\ \veczero_{(d-t)\times t} \end{bmatrix}$

\begin{enumerate}
	\item For $t = 1,2,\dots,T$
	\begin{enumerate}
		\item $\Alg$ makes a query $\query{t}$. 
		\item Draw $L_{t} \unifsim \{L \in \ortho: L^\top e_s = \query{s}, s \in [t]\}$ uniformly from the set of orthonormal matrices satisfying $L^\top\query{s} = e_s$ for $s \in [t]$. 
		\item Define the matrix $\matXtil_{t} := L_t \matX$, and denote its rows $\matxtil_{1;t},\dots,\matxtil_{d;t}$, and denote the normalized rows $\matutil_{1;t},\dots,\matutil_{d;t}$.
		\item Return the tuple $\tuple_t = (L_t, \{\|\matxtil_{s;t}\}_{s \in [t]}, \{\matutil_{s;t}\}_{s \in [t]}, \{\langle \matutil_{s;t},\matxtil_{i;t}\}_{s \in [t], i > t}\})$.
	\end{enumerate}
\end{enumerate}
\begin{lem} For all rounds $t \in [T]$ and all $s \in [t]$, (a) the queries $\matM \query{s}$ can be represented as a function of $\tuple_t$ and (b) the tuple $\tuple_s$ can be be respected as a function of the tuple $\tuple_t$.
\end{lem}
\begin{proof} We first prove point (a). Fix $t \in [T]$. Observe that for $s \in[t]$, $\matM \query{s} = \matM L_t^\top e_s = L_t^\top ( L_t \matX_t \matX_t^\top L_t^\top) e_s$, so $\matM \query{s}$ is determined by $( L_t \matX_t \matX_t^\top L_t^\top)e_s = \matXtil_t \matXtil_t^\top e_s$ and $L_t$. 
% 
Moreover, for $s \in [t]$, the vector $w_{s;t} := \matXtil_t \matXtil_t^\top e_s$ is the vector with $w_{s;t}[i] = \langle \matxtil_{t;s},\matxtil_{t;i} \rangle$. Hence, the vectors $\{w_{s;t}, s \in [t]\}$ are determined by  $(\|\matxtil\|_{s;t})_{s \in [t]})$, $(\matutil_{t;s})_{s \in [t]}$, and $(\langle\matutil_{s;t},\matxtil_{t;i} \rangle)_{s \in [t], i  > t}$. 


\end{proof}


\begin{cor}\label{cor:TW} For any $p \in (0,1)$ exists constants $C_1(p)$ and $C_2(p)$ and $d_0(p) \ge C_1(p)^{3/2} $such that, for all $d \ge d_0$

\end{cor}
We are now ready to prove Proposition~\ref{prop:testing}

\begin{proof}[Proof of Proposition~\ref{prop:testing}] Let $\matW = \matW^{(d)}$ of simplicity. Then if $\Alg$ is $\epsilon,\nu,\delta$ for $\nu \ge (C_2(p)d^{-2/3})^{-1}$,
\begin{align*}
&\Pr_{\matW,\Alg}[\lamhat \le (1+\epsilon) 2 + d^{-2/3}C_1(p)] \\
&\ge \Pr_{\matW,\Alg}[\lambda_1(\matW) \ge 2 + d^{-2/3}C_1(p) \wedge \gap(\matW) \ge \nu] - \delta \ge 1 - p- \delta.
\end{align*}
On the other hand, 
\begin{align*}
&\Pr_{\gamma\matW,\Alg}[\lamhat \ge (1-\epsilon)\cdot\gamma(2 - d^{-2/3}C_1(p)) ] \\
&\ge \Pr_{\gamma\matW,\Alg}[\{\lambda_1(\gamma\matW)(1-\epsilon) \ge (1-\epsilon)\cdot \gamma(2 - d^{-2/3}C_1(p))\} \wedge \gap(\gamma\matW) \ge \nu] - \delta\\
&= \Pr_{\gamma\matW,\Alg}[\{\lambda_1(\matW) \ge 2 - d^{-2/3}C_1(p)\} \wedge \gap(\matW) \ge \nu] - \delta \ge 1 - p - \delta,
\end{align*}
where in the last equality we use $\lambda_1(\gamma\matW) = \gamma \lambda_1(\matW)$ and $\gap(\gamma \matW) = \gap(\matW)$. Note that if $\gamma$ satisfies
\begin{align}\label{eq:gamma_condition}
(2 - d^{-2/3}C_1(p))^2 \gamma = (1-\epsilon)\gamma(2 - d^{-2/3}C_1(p))  > 2 + d^{-2/3}C_1(p),
\end{align}
 then set $\psi = \I(\xhat > (2 - d^{-2/3}C_1(p))]$ satisfies~\eqref{test_eq}. Finally, bounding $(2 - d^{-2/3}C_1(p))^2 \ge 4($
\end{proof}

Finally, we can conclude 
\begin{proof}[Proof of Theorem~\ref{thm:eigenvalue}]
\end{proof}


\subsection{Proof of Corollary~\ref{cor:TW}}
 By rescaling $p$, it suffices to show that ~\eqref{eq:stuff} holds with $1-3p$ instead of $1-p$. Let $\TWlaw$ denote the distribution from Theorem [], and consider $(X_1,X_2) \sim \TWlaw$. Since $\calD$ is a proper distribution, there exists a constant $C_1(p)$ for which $\Pr_{\TWlaw}[|X_1| \le C_1(p)] \ge 1 - p$. Moreover, since $\calD$ is absolutely continuous with respect to the Lebesgue measure, so its the distribution of $X_1 - X_2$, and therefore there exists a constant $C_2(p)$ such that $\Pr[|X_1-X_2| \ge 3C_2(p)] \ge p$. Let $A(p) \subset \R^d: \{(X_1,X_2): |X_1| \le C_1(p), |X_2| \ge 3C_2(p)\}$. Then, by a union bound have established $\Pr[(X_1,X_2) \in A(p)] \ge 1-2p$. 

Now, let $\calD^{(d)}$ denote the joint distribution of $(X_1^{(d)},X_2^{(d)}) := (d^{2/3}(\lambda_2(\matW^{(d)}) - 2,\lambda_2(\matW^{(d)})$.
Since $\TWlaw$ is continuous with respect to the Lebesgue measure, the Borel set $A$ is a continuity set of $\TWlaw$, and therefore by Theorem~\ref{thm:tw}, $\lim_{d \to\infty} \Pr_{\calD^{(d)}}[(X_1^{(d)},X_2^{(d)}) \in A(p)] = \Pr_{\TWlaw}[(X_1,X_2) \in A(p)] \ge 1- 2p$. By the definition of a limit, this means that for all $d \ge \widetilde{d}_0(p)$, $Pr_{\calD^{(d)}}[(X_1^{(d)},X_2^{(d)}) \in A(p)] \ge 1 - 3p $. 
Lastly, we show the event in~\eqref{eq:stuff} holds whenever for $(X_1^{(d)},X_2^{(d)}) \in A(p)$. Indeed, $(X_1^{(d)},X_2^{(d)}) \in A(p)$ implies $|\lambda_1(\matW) - 2| \le d^{-2/3}C_1(p)$. Further, let $d_0(p) =\widetilde{d}_0(p) \vee C_1(p)^{3/2}$, we have that $(X_1^{(d)},X_2^{(d)}) \in A(p)$ implies
\begin{align*}
\gap(\matW) = \frac{\lambda_1(\matW^{(d)}) - \lambda_2(\matW^{(d)})}{\lambda_1(\matW^{(d)})} \ge \frac{\lambda_1 - \lambda_2}{3} \ge \frac{d^{-2/3}3C_2(p)}{3} = d^{-2/3}C_2(p),
\end{align*}
as needed.




==> wishart_old.tex <==

\begin{prop}
Let $\hat{\lambda}$ be the estimate of $\lambda_{\min}(\matX\matX^\top)$ output by the algorithm. Then for any $t_1, t_2 \in \R$ with $t_1 < t_2$,
\begin{multline*}
\Pr\bracks{\lambda_{\min}(\matX\matX^\top) \leq t_1 < t_2 \leq \hat{\lambda}\,\middle|\,\vsf^{(t)}=v^{(t)},\wsf^{(t)}=w^{(t)}\ \forall t \leq T} 
\\
\geq \Pr\bracks{\hat{\lambda}\geq t_2\,\middle|\,\vsf^{(t)}=v^{(t)},\wsf^{(t)}=w^{(t)}\ \forall t \leq T} \Pr\bracks{\lambda_{\min}(W) \leq t_1}
\end{multline*}
\end{prop}
\begin{proof}
Our goal will be to identify a component of the random matrix $\matX\matX^\top$ which is independent of the $T$ queries made by the algorithm. We will later argue that failing to estimate the minimum eigenvalue of this independent component will cause the algorithm to fail with significant probability until $T = \Omega(d)$.

By Lemma \ref{lem:independent-component}, there is a rotation matrix $\matV$ such that 
\begin{equation*}
\matV\matX\matX^\top\matV^\top =
\begin{bmatrix}
Y_1Y_1^\top & Y_1Y_2^\top \\
Y_2Y_1^\top & Y_2Y_2^\top + W
\end{bmatrix}
\end{equation*}
where $W \sim \Wishart(d-T)$ conditioned on the $T$ queries and responses. This is important because, by Lemma \ref{lem:eigenvalue-of-independent-component}, $\lambda_{\min}(\matX\matX^\top) = \lambda_{\min}(\matV\matX\matX^\top\matV^\top) \leq \lambda_{\min}(W)$. The conditional independence between $W$ and the observations completes the proof.
\end{proof}










\begin{prop} Consider thresholds $0 < t_1 < t_2$, a
\begin{align*}
\Pr_{\Alg,\matM}\left[\lambda_{\min}(\matX\matX^\top) \le t_1 < t_2 \le \lamhat \right] \ge \Pr_{\Alg,\matM}\left[\lamhat \ge t_2\right] \cdot \Pr\left[ \lambda_{\min}(\matM^{(d-T)}) \le \left(\tfrac{d-T}{d}\right) t_1 \right],
\end{align*}
where $\matM^{(d-T)} \sim \Wishart(d)$. 
\end{prop}
\begin{proof}
The goal is will be to construct a matrix $\matY$, with lower-right block $\matY_{22} \in \R^{(d-T) \times (d-T)}$ such that (a) conditioned on the queries of $\Alg$, $\matY_{22}\matY_{22}^\top \sim \Wishart(d)$, and (b) with probability $1$, $\lambda_{\min}(\matY_{22}\matY_{22}^\top) \ge \lambda_{\min}(\matM) \ge \lambda_{\min}(\matX\matX^\top)$. We begin with a lemma that lets us replace conditioning on adaptive queries with conditioning for fixed queries:

\begin{claim} Fix an orthornomal set of vectors $v^{(1)},\dots,v^{(T)}$, and $w^{(1)},\dots,w^{(T)} \in \R^d$, and fix an orthonormal matrix $U$ satisfying $U^\top e_s = v^{(s)}$ for $s \in[T]$. Then, The event $\bigcap_{s = 1}^T \{\vsf^{(s)} = v^{(s)}\}\cap \bigcap_{s = 1}^T \{\wsf^{(s)} = w^{(s)}\}$ is equal to the event  $\bigcap_{s = 1}^T\{\matXtil\matXtil^\top e_s = \wtil^{(s)}\}$, where $\matXtil = U \matX $ and $\wtil^{(s)} = U w^{(s)}$. 
\end{claim}
Next, let $\matxtil_1,\dots,\matxtil_d$ denote the rows of $\matXtil$, let $\mato_1,\dots,\mato_T$ denote the Grahm-Schdmit basis for $\matxtil_1,\dots,\matxtil_T$, let $\matO = [\mato_1,\dots,\mato_T]$, and let $\matR$ be a rotation matrix drawn uniformly from the set of orthonormal matrices with $\matR[:,1:T] = \matO$. Note then that
\begin{align*}
\matY := U \matX \matR = \matXtil\matR = \begin{bmatrix} \matY_{11} & \veczero_{T \times T-d}\\
\matY_{21} & \matY_{22}
\end{bmatrix},
\end{align*}
where $\matY_{11} \in \R^{d \times d}$ is a lower triangular matrix. We shall now show $\matY_{22}$ is our desired matrix.
\begin{claim} $\sigma_{\min}(\matY) \le \sigma_{\min}(\matY_{22})$. Hence, $\lambda_{\min}(\matY_{22}\matY_{22}^\top) \ge \lambda_{\min}(\matM)$.
\end{claim}
\begin{proof} We may assume without loss of generality that $\matY_{11}$ is invertible. Let $u \in \mathcal{S}^{(T-d)-1}$ be a minimal right-singular vector of $\matY_{22}$, and let $v = \matY_{11}^{-\top}\matY_{21}^\top u$. Then
\begin{align*}
(v,u)^\top \matY = (-u^\top \matY_{21} \matY_{11}^{-1} \matY_{11} + u^\top\matY_{21},u^\top \matY_{22}) = (0, u^\top \matY_{22}).
\end{align*}
Hence,
\begin{align*}
\sigma_{\min}(\matY) \le \frac{\|(v,u)^\top \matY\|}{\|(v,u)\|} \le \frac{\|(v,u)^\top \matY\|}{\|u\|} = \frac{\|u^\top \matY_{22}\|}{\|u\|} = \sigma_{\min}(\matY_{22}).
\end{align*}
To conclude, the above implies
\begin{align*}
\lambda_{\min}(\matY_{22}\matY_{22}^\top) \le \lambda_{\min}(\matY\matY^\top) =   \lambda_{\min}(U\matX \matR \matR^\top \matX^\top U^\top) = \lambda_{\min}(\matX \matX^\top) = \lambda_{\min}(\matM),
\end{align*} where the second to last equality uses $\matY\matR^\top = I$ and that conjugating by the orthonormal matrix $U$ does not affect $\lambda_{\min}$.
\end{proof}


\begin{claim} Conditioned on $\{\matXtil\matXtil^\top e_s\}_{s \in [T]}$, $\frac{d}{d-T}\matY_{22} \matY_{22}^\top \sim \Wishart(d-T)$. 
\end{claim}

\end{proof}

\begin{claim} The matrix $\matXtil (I - \matO \matO^\top)$ is independent of the random variables. 
\end{claim}





\begin{comment}
\begin{lem} For a dimension $d$, Any matrix-vector query algorithm which makes $T < d$ queries to $\matLam := \matX^{(d)}\matX^{(d)\top}$ can be simulated in distribution from overview the first $T$ rows of $\matX$, $\matx_1,\dots,\matx_{T}$, and $\langle\matx_{i},\matx_j\rangle$ for $i \in [T]$ and $j \in [d] \setminus [T]$.
\end{lem}
\newcommand{\unit}{\mathsf{unit}}




\begin{proof} Let $\mathsf{v}^{(1)},\dots,\mathsf{v}^{(T)}$ denote the querys of $\Alg$. By Grahm-Schmidt, we may assume without loss of generality that the queries are orthonormal. Moreover, since the distribution of $\matLam$ is rotation-invariant, we may assume without loss of generality that $\mathsf{v}^{(1)} = e_1$, the first cannonical basis vector. Then, $\matLam\mathsf{v}^{(1)} = (\|\matx_1\|^2, \langle \matx_1,\matx_2 \rangle,\dots \langle \matx_1,\matx_d)$. This query can be simulated by a stronger oracle which provides $\matx_1$, and letting $\unit(\matx_1) := \matx_1/\|\matx_1\|$, provides $\langle \unit(\matx_1),\matx_2 \rangle,\dots \langle \unit(\matx_1),\matx_d)$. 

Now, let $O_1$ denote any rotation matrice for which $O^\top \unit(\matx_1) = e_1$, i.e. the first row of $O^{\top}$ is equal to $\unit(\matx_1)$. and let $\matX^{(d,1)} := \matX^{(d)}O_1$. Then, $ \matX^{(d,1)} $ has the form
\begin{align*}
\matX^{(d,1)} = \begin{bmatrix} \|\matx_1\| & \mathbf{0}_{1 \times d- 1} \\
 \matX^{(d)}[2:d,:]^\top \matx_1 & O_1[2:d,2:d] \cdot \matX^{(d)}[2:d,2:d]  \end{bmatrix}
\end{align*}
Now, since $\matX^{(d,1)}$ is related to $\matX^{(d)}$ 
\end{proof}
\end{comment}
